RetrieveGAN: Image Synthesis via Differentiable Patch Retrieval

Image generation from scene description is a cornerstone technique for the controlled generation, which is beneficial to applications such as content creation and image editing. In this work, we aim to synthesize images from scene description with retrieved patches as reference. We propose a differentiable retrieval module. With the differentiable retrieval module, we can (1) make the entire pipeline end-to-end trainable, enabling the learning of better feature embedding for retrieval; (2) encourage the selection of mutually compatible patches with additional objective functions. We conduct extensive quantitative and qualitative experiments to demonstrate that the proposed method can generate realistic and diverse images, where the retrieved patches are reasonable and mutually compatible.

==> table/dataset.tex <==
\begin{table*}[t]
    \setlength{\tabcolsep}{4pt}
        \caption{\textbf{Statistics of datasets.} 
    }
    \label{tab:dataset}
    \centering
    \begin{tabular}{l c c c c c } 
	    \toprule
		Dataset & Train & Val & Test & $\#$ Category & $\#$ Patches \\
		\midrule
		COCO-Stuff & 74121 & 1024& 2048& 171& 411682\\
		Visual Genome & 62565& 5506 & 5088 & 178 & 606319\\
		\bottomrule
    \end{tabular}

    \vspace{\tabmargin}
\end{table*}
